Adversarial Feature Map Pruning for Backdoor

Deep neural networks have been widely used in many critical applications, such as autonomous vehicles and medical diagnosis. However, their security is threatened by backdoor attacks, which are achieved by adding artificial patterns to specific training data. Existing defense strategies primarily focus on using reverse engineering to reproduce the backdoor trigger generated by attackers and subsequently repair the DNN model by adding the trigger into inputs and fine-tuning the model with ground-truth labels. However, once the trigger generated by the attackers is complex and invisible, the defender cannot reproduce the trigger successfully then the DNN model will not be repaired, as the trigger is not effectively removed. In this work, we propose Adversarial Feature Map Pruning for Backdoor (FMP) to mitigate backdoor from the DNN. Unlike existing defense strategies, which focus on reproducing backdoor triggers, FMP attempts to prune backdoor feature maps, which are trained to extract backdoor information from inputs. After pruning these backdoor feature maps, FMP will fine-tune the model with a secure subset of training data. Our experiments demonstrate that, compared to existing defense strategies, FMP can effectively reduce the Attack Success Rate (ASR) even against the most complex and invisible attack triggers (e.g., FMP decreases the ASR to 2.86\% in CIFAR10, which is 19.2\% to 65.41\% lower than baselines). Second, unlike conventional defense methods that tend to exhibit low robust accuracy (that is, the accuracy of the model on poisoned data), FMP achieves a higher RA, indicating its superiority in maintaining model performance while mitigating the effects of backdoor attacks (e.g., FMP obtains 87.40\% RA in CIFAR10). Our code is publicly available at: https://github.com/retsuh-bqw/FMP.

==> background.tex <==
\section{background}
In this section,  we will define backdoor and then discuss three classical real-world scenarios in which backdoor attacks may occur.
\subsection{Defining Backdoors.} 

We define a DNN backdoor to be a hidden pattern trained into a DNN, which produces unexpected behavior if and only if a specific trigger is added to an input. Such a backdoor does not affect the model’s normal behavior on clean inputs without the trigger. In the context of classification tasks, a backdoor misclassifies arbitrary inputs into the same specific target label, when the associated trigger is applied to inputs. Input samples that should be classified into any other label could be “overridden” by the presence of the trigger. In the vision domain, a trigger is often a specific pattern on the image (e.g., a sticker), that could misclassify images of other labels (e.g., wolf, bird, dolphin) into the target label (e.g., dog).



\subsection{Backdoor Attack Scenarios and Capacities}

To analyze the challenges and complexities associated with backdoor attacks in deep learning, we outline three classical real-world scenarios where such threats can occur, along with the corresponding capacities available to attackers and defenders. By examining these scenarios, we aim to provide a thorough understanding of the risks associated with backdoor attacks and the necessity for effective defense mechanisms.

\subsubsection{Scenario 1: Adopting Third-Party Datasets}

In this scenario, developers rely on third-party-provided datasets~(e.g., DataTurks~\cite{dataturks}), either directly or via the Internet, to train their models. This dependence on external data sources increases the risk of backdoor attacks since the attacker can manipulate the dataset to inject subtle triggers. However, they cannot modify the model, training schedule, or inference pipeline, which limits their ability to control the system. Conversely, defenders have full control over the system and can take various measures to mitigate the backdoor threat. For instance, they can clean up the poisoned dataset, implement data augmentation strategies, or use anomaly detection techniques to identify and remove potential triggers.

\subsubsection{Scenario 2: Adopting Third-Party Platforms}

In this scenario, developers use untrusted third-party platforms (e.g., Google Cloud~\cite{google_cloud}, AWS Cloud~\cite{aws}, or HUAWEI Cloud~\cite{huawei_cloud}) to train their models, providing the platform with a benign dataset, model structure, and training schedule. The attacker (i.e., the malicious platform) can modify the dataset and training schedule during the actual training process, but they cannot change the model structure, as the developers would notice. This limitation requires the attacker to be more stealthy and sophisticated in their approach. On the other hand, defenders cannot control the training set and schedule, but they can modify the trained model to alleviate the attack, such as by fine-tuning it on a small local benign dataset or using techniques like knowledge distillation to transfer knowledge from the compromised model to a new, clean model.

\subsubsection{Scenario 3: Adopting Third-Party Models}

In this scenario, attackers provide infected DNNs through APIs or the Internet (e.g., Hugging Face~\cite{huggingface}). They can modify everything except for the inference pipeline, which means developers can introduce a pre-processing module on the test image before prediction, out of the attackers' control. This constraint forces attackers to craft more advanced and persistent backdoors that can survive such pre-processing. Defenders can control the inference pipeline and the model if its source files are provided. However, if they can only access the model API, they cannot modify the model directly. In this case, defenders must resort to techniques like input validation, or reverse engineering to detect and mitigate the backdoor threat.

% In summary, the attacker's capacities increase while the defender's capacities decrease from Scenario 1 to Scenario 3. Consequently, attacks designed for a previous scenario could also occur in subsequent scenarios, but they may require adaptations to accommodate the additional constraints. Likewise, defenses designed for a later scenario could be applied to previous ones, but they may need to be fine-tuned to address the specific risks associated with each scenario. By delving into these scenarios, we can better understand the growing risks associated with backdoor attacks and develop more robust and adaptive defense mechanisms to ensure the security and trustworthiness of deep learning models.

% In this work, we discussion DNN developer under 1-th and 2-nd scenario, i.e., DNN developer only have few security dataset so they need download third party dataset and upload it to third party platforms.


